Wireless Microwave Quantum Communication

This Thesis explores the limits in the application of propagating quantum microwaves for quantum communication and quantum sensing, as well as the design of new devices and protocols to fight these limitations. We take advantage of Gaussian quantum states for quantum teleportation and quantum illumination, and studies how these protocols can be improved using entanglement distillation and partial purification, respectively. The Thesis is centered around open-air entanglement distribution, and it follows the steps of state generation inside the cryostat, impedance matching between the cryostat and the open air with a new generation of coplanar antennae, and open air propagation, in the limited framework of current microwave technology. We also address the limitations produced by losses and measurement inefficiencies, and explore the extension to satellite quantum communications. There, we analyze the effects of diffraction and turbulence, studying how the latter affects signals in the optical regime as well. We conclude by studying the teleportation of quantum information in a quantum local area network. To sum up, this Thesis contributes to the development of wireless quantum communications in the microwave regime, studying its technological limitations and how to overcome them. Nevertheless, quantum technologies working in this frequency range are still emergent and plenty of work must be accomplished in order to make them competitive.

==> snp/fancySection3.tex <==
% \titleformat{\section}[display]
% {\vspace*{150pt}
% \bf\Huge}
% {\hspace{-72pt}{\textcolor{grey}{\thesection}} \hspace{38pt} {\textcolor{white}{#1}}}
% {0pt}
% {}
% []
% \titlespacing*{\section}{108pt}{10pt}{60pt}[20pt]
%
% %Intro
% \titleformat{\section}[display]
% {\vspace*{190pt}
% \bfseries\sffamily \huge}
% {\begin{picture}(0,0)\put(-50,-25){\textcolor{grey}{\thesection}}\end{picture}}
% {0pt}
% {\textcolor{white}{#1}}
% []
% \titlespacing*{\section}{80pt}{10pt}{50pt}[20pt]
%
% %ch 2
% \titleformat{\section}[display]
% {\vspace*{190pt}
% \bfseries\sffamily \huge}
% {\begin{picture}(0,0)\put(-50,-28){\textcolor{grey}{\thesection}}\end{picture}}
% {0pt}
% {\textcolor{white}{#1}}
% []
% \titlespacing*{\section}{80pt}{10pt}{50pt}[20pt]
%
% %ch 3, 4 y 5
\titleformat{\section}[display]
{\vspace*{150pt}
\bfseries\sffamily \LARGE}
{\begin{picture}(0,0)\put(-50,-44){\textcolor{grey}{\thesection}}\end{picture}}
{-25pt}
{\textcolor{white}{#1}}
[]
\titlespacing*{\section}{80pt}{10pt}{40pt}[20pt]
%\titlespacing*{\section}{80pt}{10pt}{40pt}[20pt]

% %Conclusions
% %Julen conclusions
% \titleformat{\section}[display]
% {\vspace*{190pt}
% \bfseries\sffamily \huge}
% {\begin{picture}(0,0)\put(-50,-25){\textcolor{grey}{\thesection}}\end{picture}}
% {0pt}
% {\textcolor{white}{#1}}
% []
% \titlespacing*{\section}{80pt}{10pt}{50pt}[20pt]


==> snp/fancySection6.tex <==
% \titleformat{\section}[display]
% {\vspace*{150pt}
% \bf\Huge}
% {\hspace{-72pt}{\textcolor{grey}{\thesection}} \hspace{38pt} {\textcolor{white}{#1}}}
% {0pt}
% {}
% []
% \titlespacing*{\section}{108pt}{10pt}{60pt}[20pt]
%
% %Intro
% \titleformat{\section}[display]
% {\vspace*{190pt}
% \bfseries\sffamily \huge}
% {\begin{picture}(0,0)\put(-50,-25){\textcolor{grey}{\thesection}}\end{picture}}
% {0pt}
% {\textcolor{white}{#1}}
% []
% \titlespacing*{\section}{80pt}{10pt}{50pt}[20pt]
%
% %ch 2
% \titleformat{\section}[display]
% {\vspace*{190pt}
% \bfseries\sffamily \huge}
% {\begin{picture}(0,0)\put(-50,-28){\textcolor{grey}{\thesection}}\end{picture}}
% {0pt}
% {\textcolor{white}{#1}}
% []
% \titlespacing*{\section}{80pt}{10pt}{50pt}[20pt]
%
% %ch 3, 4 y 5
\titleformat{\section}[display]
{\vspace*{190pt}
\bfseries\sffamily \huge}
{\begin{picture}(0,0)\put(-50,-25){\textcolor{grey}{\thesection}}\end{picture}}
{0pt}
{\textcolor{white}{#1}}
[]
\titlespacing*{\section}{80pt}{10pt}{50pt}[20pt]
%\titlespacing*{\section}{80pt}{10pt}{40pt}[20pt]

% %Conclusions
% %Julen conclusions
% \titleformat{\section}[display]
% {\vspace*{190pt}
% \bfseries\sffamily \huge}
% {\begin{picture}(0,0)\put(-50,-25){\textcolor{grey}{\thesection}}\end{picture}}
% {0pt}
% {\textcolor{white}{#1}}
% []
% \titlespacing*{\section}{80pt}{10pt}{50pt}[20pt]

